Hierarchical Temporal Point Process Modeling of Aggressive Behavior Onset in Psychiatric Inpatient Youth with Autism for Branching Factor Estimation

Aggressive behavior in autistic inpatient youth often arises in temporally clustered bursts complicating efforts to distinguish external triggers from internal escalation. The sample population branching factor-the expected number of new onsets triggered by a given event-is a key summary of self-excitation in behavior dynamics. Prior pooled models overestimate this quantity by ignoring patient-specific variability. We addressed this using a hierarchical Hawkes process with an exponential kernel and edge-effect correction allowing partial pooling across patients. This approach reduces bias from high-frequency individuals and stabilizes estimates for those with sparse data. Bayesian inference was performed using the No U-Turn Sampler with model evaluation via convergence diagnostics, power-scaling sensitivity analysis, and multiple Goodness-of-Fit (GOF) metrics: PSIS-LOO the Lewis test with Durbin's modification and residual analysis based on the Random Time Change Theorem (RTCT). The hierarchical model yielded a significantly lower and more precise branching factor estimate mean (0.742 +- 0.026) than the pooled model (0.899 +- 0.015) and narrower intervals than the unpooled model (0.717 +- 0.139). This led to a threefold smaller cascade of events per onset under the hierarchical model. Sensitivity analyses confirmed robustness to prior and likelihood perturbations while the unpooled model showed instability for sparse individuals. GOF measures consistently favored or on par to the hierarchical model. Hierarchical Hawkes modeling with edge-effect correction provides robust estimation of branching dynamics by capturing both within- and between-patient variability. This enables clearer separation of endogenous from exogenous events supports linkage to physiological signals and enhances early warning systems individualized treatment and resource allocation in inpatient care.

==> figure_caption_sheet.tex <==
% Figure Captions Sheet
\begin{center}
    \textbf{Figure Captions}
\end{center}

\newcounter{savefigure2}

% Start of your special section
\setcounter{savefigure2}{\value{figure}}  % Save current figure number
\setcounter{figure}{0}    

\begin{flushleft}
\noindent \textit{Figure 1.} Hierarchical model structure for partially pooled Hawkes process.

\noindent \textit{Figure 2.} Branching factor estimates for pooled, unpooled, and partially pooled models. The partially pooled model has a statistically significantly lower mean than the pooled model, with a substantially lower uncertainty than the unpooled model.

\noindent \textit{Figure 3.} Expected total number of subsequent aggressive behavior onsets (descendants) triggered by a single parent onset, comparing pooled and partially pooled models.

\noindent \textit{Figure 4.} Branching factor estimates for the unpooled and partially pooled models after various power-scale perturbations in the prior. The unpooled model's branching factor estimates are highly sensitive to prior perturbations, while the partially pooled model's estimates remain stable across power-scale perturbations.

\noindent \textit{Figure 5.} Examples of inferred branching structures (first row of each subfigure) and probability of exogenous event (second row of each subfigure) for six observation sessions. (a) Session 131, (b) Session 77, (c) Session 95, (d) Session 62, (e) Session 40 and (g) Session 41. Green circles indicate endogenous events triggered by the edge effect, light blue circles represent child (offspring) events from subsequent generations, and green squares denote parent (exogenous) events. Magenta x's mark the observed aggressive behavior onset times (point data). The shaded area in the probability of onset being exogenous if occuring at time $t$ is the highest density interval from the posterior distribution. In the physiological signals, the shaded red line indicates aggressive behavior (not just the onset, but the continued behavior). The timeline is in minutes.

% \noindent \textit{Figure 6.} Q-Q plot of the RTCT inter-arrival times of aggressive behavior onsets for a sample patient. The plot compares the empirical quantiles of the inter-arrival times to the theoretical quantiles of the unit-rate exponential distribution. The points closely follow the diagonal line, indicating that the inter-arrival times follow a unit-rate exponential distribution.

% \noindent \textit{Figure 7.} Scatter plot of the uniform-transformed \gls{rtct} inter-arrival times for observation sessions with more than 5 aggressive behavior onsets. The plot shows the relationship between the uniform-transformed inter-arrival times at lag 1 and lag 2. The points are randomly scattered, indicating that the inter-arrival times are independent and identically distributed.
\end{flushleft}



\pagebreak

\begin{figure}[h!]
    \centering
    \captionsetup{style=special}  % apply special caption style here only
    \caption{}
    \input{images/hierarchical-pgm}
\end{figure}

\pagebreak

\begin{figure}[h!]
    \centering
    \captionsetup{style=special}  % apply special caption style here only
    \caption{}
    \includegraphics[width=0.9\textwidth]{images/plot_branching_factor_distribution_overlapped.pdf}
\end{figure}

\pagebreak

\begin{figure}[h!]
    \centering
    \captionsetup{style=special}  % apply special caption style here only
    \caption{}
    \includegraphics[width=0.9\linewidth]{images/plot_expected_descendent_overlapped.pdf}
\end{figure}

\pagebreak

\begin{figure}[h!]
    \centering
    \captionsetup{style=special}  % apply special caption style here only
    \caption{}
    \includegraphics[width=0.9\textwidth]{images/plot_bf_sensitivty.pdf}
\end{figure}

\pagebreak

\begin{figure}[h!]
    \centering
    \captionsetup{style=special}  % apply special caption style here only
    \caption{}
    \begin{minipage}[t]{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/branch-exogenous-structure/figure_header.png}
    \end{minipage}
    \vspace{0.5em}
    \begin{minipage}[t]{0.465\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/branch-exogenous-structure/session_id_131_all.png}
        \subcaption{Session 131 Branching Structure}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/branch-exogenous-structure/session_id_77_all.png}
        \subcaption{Session 77 Branching Structure}
    \end{minipage}
    \vspace{0.5em}
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/branch-exogenous-structure/session_id_95_all.png}
        \subcaption{Session 95 Branching Structure}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/branch-exogenous-structure/session_id_62_all.png}
        \subcaption{Session 62 Branching Structure}
    \end{minipage}
    \vspace{0.5em}
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/branch-exogenous-structure/session_id_40_all.png}
        \subcaption{Session 40 Branching Structure}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/branch-exogenous-structure/session_id_41_all.png}
        \subcaption{Session 41 Branching Structure}
    \end{minipage}
\end{figure}

% \pagebreak

% \begin{figure}[h!]
%     \centering
%     \captionsetup{style=special}  % apply special caption style here only
%     \caption{}
%     \includegraphics[width=1.0\textwidth]{images/plot_quantile_quantile.pdf}

% \end{figure}

% \pagebreak

% \begin{figure}[h!]
%     \centering
%     \captionsetup{style=special}  % apply special caption style here only
%     \caption{}
%     \includegraphics[width=1.0\textwidth, trim=0 0 0 120, clip]{images/HawkesPriorExpPP_partialpooled_plot_autocorrelation.pdf}

% \end{figure}

\pagebreak    

\begin{center}
    \textbf{Table Captions}
\end{center}

\begin{flushleft}
\noindent \textit{Table 1.} Prior/Likelihood Power Scaling Sensitivity Analysis Results for the Unpooled Model. The table shows the sensitivity of the posterior distribution over Hawkes Point Process parameters to perturbations in the prior and likelihood using the power-scaling approach. The subscript $i$ indicates the patient. The ``prior'' and ``likelihood'' columns show the cumulative Jensen-Shannon distance between the based and perturbed posterior distribution under power-scaling of the prior or likelihood, respectively. The ``diagnosis'' column indicates whether the parameter is robust (\checkmark) or shows potential sensitivity to the prior or likelihood.

\noindent \textit{Table 2.} Prior/Likelihood Power Scaling Sensitivity Analysis Results for the Partial Pooled Model. The table shows the sensitivity of the posterior distribution over population-level Hawkes Point Process parameters to perturbations in the prior and likelihood using the power-scaling approach. The ``prior'' and ``likelihood'' columns show the cumulative Jensen-Shannon distance between the based and perturbed posterior distribution under power-scaling of the prior or likelihood, respectively. The ``diagnosis'' column indicates whether the parameter is robust (\checkmark) or shows potential sensitivity to the prior or likelihood.

\noindent \textit{Table 3.} Goodness of Fit Results. The table shows the results of the Pareto-Smoothed Importance Sampling - Leave One Out Cross-Validation (PSIS-LOO-CV) Expected Log Density Prediction (ELPD) for the pooled, unpooled, and partially pooled models. The effective number of parameters (p) is also shown. The weight is calculated using stacking to estimate model preference for prediction. Estimated from 429 observation sessions.

\noindent \textit{Table 4.} Lewis test with Durbin's modification: rejection rates at various significance levels for each model. Results are reported for both session-level and patient-level analyses. For the session-level, we report the average proportion of sessions that do not reject the null hypothesis. For the patient-level analysis, we report the average proportion of patients in which the null hypothesis was rejected. Only sessions with more than 5 events were included (157 out of 429 sessions, corresponding to 39 out of 70 patients).

% \noindent \textit{Table 5.} Goodness of fit results for the two additional tests: the Independence Test (Ljung–Box test on uniform-transformed inter-arrival times) and the Marginal Exponential Test (Kolmogorov–Smirnov test on transformed inter-arrival times per patient). Results are reported as the proportion of sessions (Independence Test) and patients (Marginal Exponential Test) that do not reject the null hypothesis at various significance levels for each model. Only sessions with more than 5 events were included.

\noindent \textit{Table 5.} Goodness of fit results for the Poisson Process model. The table shows the proportion of sessions that do not reject the null hypothesis at various significance levels for the partial pooled and pooled models.

\noindent \textit{Table 6.} MCMC diagnostics for the partial pooled model parameters. The statistics are generated from 4000 MCMC samples from the posterior distribution of the model parameters Statistics are based on 4000 MCMC samples from the posterior distributions. Reported metrics include Monte Carlo standard errors (mcse), effective sample sizes (ess), and $\hat{R}$ convergence diagnostics for each parameter.

\noindent \textit{Table 7.} MCMC diagnostics for the pooled model parameters. The statistics are generated from 4000 MCMC samples from the posterior distribution of the model parameters Statistics are based on 4000 MCMC samples from the posterior distributions. Reported metrics include Monte Carlo standard errors (mcse), effective sample sizes (ess), and $\hat{R}$ convergence diagnostics for each parameter.

\noindent \textit{Table 8.} MCMC diagnostics for the unpooled model parameters. The statistics are generated from 4000 MCMC samples from the posterior distribution of the model parameters Statistics are based on 4000 MCMC samples from the posterior distributions. Reported metrics include Monte Carlo standard errors (mcse), effective sample sizes (ess), and $\hat{R}$ convergence diagnostics for each parameter.

\noindent \textit{Table 9.} Power scale analysis results for the partial pooled model hyperparameters and patient-level parameters. Each row reports the sensitivity of the posterior distribution for a parameter to power-scaling of the prior and likelihood, respectively. The ``prior'' and ``likelihood'' columns show the cumulative Jensen-Shannon distance between the based and perturbed posterior distribution under power-scaling of the prior or likelihood, respectively. The ``diagnosis'' column indicates whether the parameter is robust (\checkmark) or shows potential sensitivity to the prior or likelihood.

\noindent \textit{Table 10.} Power scale analysis results for the unpooled model hyperparameters and patient-level parameters. Each row reports the sensitivity of the posterior distribution for a parameter to power-scaling of the prior and likelihood, respectively. The ``prior'' and ``likelihood'' columns show the cumulative Jensen-Shannon distance between the based and perturbed posterior distribution under power-scaling of the prior or likelihood, respectively. The ``diagnosis'' column indicates whether the parameter is robust (\checkmark) or shows potential sensitivity to the prior or likelihood.


\end{flushleft}

% End of special section — restore original numbering
\setcounter{figure}{\value{savefigure2}}  % Restore original figure number
\renewcommand{\thefigure}{\arabic{figure}}  % Restore default figure numbering
